A Stochastic Approach to Bi-Level Optimization for Hyperparameter Optimization and Meta Learning

We tackle the general differentiable meta learning problem that is ubiquitous in modern deep learning, including hyperparameter optimization, loss function learning, few-shot learning, invariance learning and more. These problems are often formalized as Bi-Level optimizations (BLO). We introduce a novel perspective by turning a given BLO problem into a stochastic optimization, where the inner loss function becomes a smooth probability distribution, and the outer loss becomes an expected loss over the inner distribution. To solve this stochastic optimization, we adopt Stochastic Gradient Langevin Dynamics (SGLD) MCMC to sample inner distribution, and propose a recurrent algorithm to compute the MC-estimated hypergradient. Our derivation is similar to forward-mode differentiation, but we introduce a new first-order approximation that makes it feasible for large models without needing to store huge Jacobian matrices. The main benefits are two-fold: i) Our stochastic formulation takes into account uncertainty, which makes the method robust to suboptimal inner optimization or non-unique multiple inner minima due to overparametrization; ii) Compared to existing methods that often exhibit unstable behavior and hyperparameter sensitivity in practice, our method leads to considerably more reliable solutions. We demonstrate that the new approach achieves promising results on diverse meta learning problems and easily scales to learning 87M hyperparameters in the case of Vision Transformers.

==> backup/main_full_bib <==


@article{ebm1,
  title={Implicit Generation and Modeling with Energy Based Models},
  author={T. Du and I. Mordatch},
  journal={Advances in Neural Information Processing Systems},
  year={2019}
}

@article{ebm2,
  title={Your Classifier is Secretly an Energy Based Model and You Should Treat it Like One},
  author={W. Grathwohl and K. Wang and J. Jacobsen and D. Duvenaud and M. Norouzi and K. Swersky},
  journal={International Conference on Learning Representation},
  year={2020}
}

@article{bmaml,
  title={Bayesian Model-Agnostic Meta-Learning},
  author={J. Yoon and T. Kim and O. Dia and S. Kim and Y. Bengio and S. Ahn},
  journal={Advances in Neural Information Processing Systems},
  year={2018}
}

@article{abml,
  title={Amortized Bayesian Meta-Learning},
  author={S. Ravi and A. Beatson},
  journal={International Conference on Learning Representation},
  year={2019}
}

@article{calibration,
  title={On Calibration of Modern Neural Networks},
  author={Chuan Guo and Geoff Pleiss and Yu Sun and Kilian Q. Weinberger},
  journal={International Conference on Machine Learning},
  year={2017}
}



@article{ghadimi_lan,
  title={Stochastic First- and Zeroth-Order Methods for Nonconvex Stochastic Programming},
  author={Saeed Ghadimi and Guanghui Lan},
  journal={SIAM Journal on Optimization},
  volume={23},
  number={4}, 
  pages={2341--2368},
  year={2013},
}

@article{es_ns,
  title={Random Gradient-Free Minimization of Convex Functions},
  author={Y. Nesterov and V. Spokoiny},
  journal={Foundations of Computational Mathematics},
  volume={17},
  pages={527--566},
  year={2017},
  publisher={Springer}
}


@article{ghadimi18,
  title={{Approximation methods for bilevel programming}},
  author={S. Ghadimi and M. Wang},
  journal={arXiv preprint arXiv:1802.02246},
  year={2018}
}

@article{blo_naa,
  title={Bilevel optimization: Nonasymptotic analysis and faster algorithms},
  author={K. Ji and J. Yang and Y. Liang},
  journal={International Conference on Machine Learning},
  year={2021}
}



@article{storm,
  title={{Momentum-Based Variance Reduction in Non-Convex SGD}},
  author={Ashok Cutkosky and Francesco Orabona},
  journal={arXiv preprint arXiv:1905.10018},
  year={2019}
}


@article{ref_A,
  title={Provably Faster Algorithms for Bilevel Optimization},
  author={Yang, J. and Ji, K. and Liang, Y.},
  journal={Advances in Neural Information Processing Systems},
  year={2021}
}

@article{ref_B,
  title={Amortized Implicit Differentiation for Stochastic Bilevel Optimization},
  author={Arbel, M. and Mairal, J.},
  journal={International Conference on Machine Learning},
  year={2022}
}

@article{ref_C,
  title={Fully Single Loop Algorithm for Bilevel Optimization without Hessian Inverse},
  author={Li, J. and Gu, B. and Huang, H. A},
  journal={AAAI},
  year={2022}
}

@article{ref_D,
  title={A framework for bilevel optimization that enables stochastic and global variance reduction algorithms},
  author={Dagr\'{e}ou, M. and Ablin, P. and Vaiter, S. and Moreau, T.},
  journal={Advances in Neural Information Processing Systems},
  year={2023}
}



@inproceedings{alg_diff1,
  title={{Evaluating Derivatives: Principles and Techniques of Algorithmic Differentiation}},
  author={Griewank, Andreas and Walther, Andrea},
  booktitle={Society for Industrial and Applied Mathematics, Second Edition},
  year={2008}
}

@article{alg_diff2,
  title={{Automatic differentiation in machine learning: A survey}},
  author={Atilim Gunes Baydin and Barak A. Pearlmutter and Alexey Andreyevich Radul and Jeffrey Mark Siskind},
  journal={arXiv preprint arXiv:1502.05767},
  year={2015}
}



@article{blo_survey,
  title={{Gradient-based Bi-level Optimization for Deep Learning: A Survey}},
  author={Can Chen and Xi Chen and Chen Ma and Zixuan Liu and Xue Liu},
  journal={arXiv preprint arXiv:2207.11719},
  year={2022}
}


@InProceedings{pmlr-v162-yang22g,
  title = 	 {{Efficient Variance Reduction for Meta-learning}},
  author =       {Yang, Hansi and Kwok, James},
  booktitle = 	 {International Conference on Machine Learning},
  year = 	 {2022},
}

@article{liu2021investigatingBLO,
  title={Investigating bi-level optimization for learning and vision from a unified perspective: A survey and beyond},
  author={Liu, Risheng and Gao, Jiaxin and Zhang, Jin and Meng, Deyu and Lin, Zhouchen},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={12},
  pages={10045--10067},
  year={2021},
  publisher={IEEE}
}

@InProceedings{meta_inr,
  author = {Matthew Tancik and Ben Mildenhall and Terrance Wang and Divi Schmidt and Pratul P. Srinivasan and Jonathan T. Barron and Ren Ng},
  title = {Learned Initializations for Optimizing Coordinate-Based Neural Representations},
  booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year = {2021}
}




@Book{mcmc_book,
  author = 	 "Dani Gamerman and Hedibert F. Lopes",
  title = 	 "Markov Chain Monte Carlo: Stochastic Simulation for Bayesian Inference",
  publisher = 	 "Chapman \& Hall/CRC Texts in Statistical Science",
  year = 	 "2006",
}


@inproceedings{imaml,
  title={{Meta-Learning with Implicit Gradients}},
  author={Aravind Rajeswaran and Chelsea Finn and Sham Kakade and Sergey Levine},
  booktitle={Advances in Neural Information Processing Systems},
  year={2019}
}

@InProceedings{luketina2016scalableRegularization,
  author    = {Jelena Luketina and Mathias Berglund and Klaus Greff and Tapani Raiko},
  title     = {Scalable Gradient-Based Tuning of Continuous Regularization Hyperparameters},
  booktitle = {ICML},
  year      = {2016},
}

@article{micaelli2021gradient,
  title={Gradient-based hyperparameter optimization over long horizons},
  author={Micaelli, Paul and Storkey, Amos J},
  journal={Advances in Neural Information Processing Systems},
  year={2021}
}

@inproceedings{metz2019understanding,
  title={Understanding and correcting pathologies in the training of learned optimizers},
  author={Metz, Luke and Maheswaranathan, Niru and Nixon, Jeremy and Freeman, Daniel and Sohl-Dickstein, Jascha},
  booktitle={International Conference on Machine Learning},
  year={2019},
}

@InProceedings{fmd_rmd,
  title = 	 {{Forward and Reverse Gradient-Based Hyperparameter Optimization}},
  author =       {Luca Franceschi and Michele Donini and Paolo Frasconi and Massimiliano Pontil},
  booktitle = 	 {International Conference on Machine Learning},
  year = 	 {2017},
}
@InProceedings{lorraine2020optimizing,
  author       = {Lorraine, Jonathan and Vicol, Paul and Duvenaud, David},
  booktitle    = {International Conference on Artificial Intelligence and Statistics},
  title        = {Optimizing millions of hyperparameters by implicit differentiation},
  year         = {2020},
}

@article{taylorglo,
	author = {Gonzalez, Santiago and Miikkulainen, Risto},
	year = {2021},
	month = {07},
	pages = {},
	title = {Optimizing Loss Functions Through Multivariate Taylor Polynomial Parameterization},
	journal = {Proceedings of the Genetic and Evolutionary Computation Conference (GECCO-2021)}
}

@article{vit,
  title={{An image is worth 16x16 words: Transformers for image recognition at scale}},
  author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@article{reinforce,
  title={{Simple statistical gradient-following algorithms for connectionist reinforcement learning}},
  author={Ronald J. Williams},
  journal={Machine Learning},
  year={1992},
  volume = {8},
  pages = {229--256}
}

@InProceedings{dtd,
  Author    = {M. Cimpoi and S. Maji and I. Kokkinos and S. Mohamed and and A. Vedaldi},
	 Title     = {Describing Textures in the Wild},
	 Booktitle = {Proceedings of the {IEEE} Conf. on Computer Vision and Pattern Recognition ({CVPR})},
  Year      = {2014}
}


@InProceedings{overparam_blo,
  title = 	 {{On Implicit Bias in Overparameterized Bilevel Optimization}},
  author =       {Vicol, Paul and Lorraine, Jonathan P and Pedregosa, Fabian and Duvenaud, David and Grosse, Roger B},
  booktitle = 	 {International Conference on Machine Learning},
  year = 	 {2022},
}


@inproceedings{hpo_partition,
 title = {{Hyperparameter Optimization through Neural Network Partitioning}},
 author  = {Bruno Kacper Mlodozeniec and Matthias Reisser and Christos Louizos},
 year  = {2023},
 booktitle = {International Conference on Learning Representations}
}


@inproceedings{lila,
  title={{Invariance Learning in Deep Neural Networks with Differentiable Laplace Approximations}},
  author={Alexander Immer and Tycho F.A. van der Ouderaa and Vincent Fortuin and Gunnar R\"{a}tsch and Mark van der Wilk},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022}
}

@inproceedings{augerino,
  title={{Learning Invariances in Neural Networks}},
  author={Gregory Benton and Marc Finzi and Pavel Izmailov and Andrew Gordon Wilson},
  booktitle={Advances in Neural Information Processing Systems},
  year={2020}
}



@misc{ift,
 author = {Jonathan Lorraine and Paul Vicol and David Duvenaud},
 title = {{Optimizing Millions of Hyperparameters by Implicit Differentiation}},
 note = {AI and Statistics (AISTATS)},
 year = 2020
}


@inproceedings{clml,
 title = {{Bayesian Model Selection, the Marginal Likelihood, and Generalization}},
 author  = {Sanae Lotfi and Pavel Izmailov and Gregory Benton and Micah Goldblum and Andrew Gordon Wilson},
 year  = {2022},
 booktitle = {International Conference on Machine Learning}
}


@inproceedings{sgld,
 title = {{Bayesian Learning via Stochastic Gradient Langevin Dynamics}},
 author  = {Max Welling and Yee Whye Teh},
 year  = {2011},
 booktitle = {International Conference on Machine Learning}
}

@inproceedings{swa,
  title={{Averaging weights leads to wider optima and better generalization}},
  author={Pavel Izmailov and Dmitrii Podoprikhin and Timur Garipov and Dmitry Vetrov and Andrew Gordon Wilson},
  booktitle={Uncertainty in Artificial Intelligence},
  year={2018}
}

@article{swag,
  title={{A Simple Baseline for Bayesian Uncertainty in Deep Learning}},
  author={Wesley Maddox and Timur Garipov and Pavel Izmailov and Dmitry Vetrov and Andrew Gordon Wilson},
  journal={arXiv preprint arXiv:1902.02476},
  year={2019}
}

@article{shapenet,
  title={{ShapeNet: An Information-Rich 3D Model Repository}},
  author={Angel X. Chang and Thomas Funkhouser and Leonidas Guibas and Pat Hanrahan and Qixing Huang and Zimo Li and Silvio Savarese and Manolis Savva and Shuran Song and Hao Su and Jianxiong Xiao and Li Yi and Fisher Yu},
  journal={arXiv preprint arXiv:1512.03012},
  year={2015}
}




@inproceedings{simplified_nerf,
 title = {{NeRF: Representing scenes as neural radiance fields for view synthesis}},
 author  = {Ben Mildenhall and Pratul P. Srinivasan and Matthew Tancik and Jonathan T. Barron and Ravi Ramamoorthi and Ren Ng.},
 year  = {2020},
 booktitle = {European Conference on Computer Vision}
}


@inproceedings{mc_dropout,
 title = {{Dropout as a Bayesian Approximation: Representing Model Uncertainty in Deep Learning}},
 author  = {Yarin Gal and Zoubin Ghahramani},
 year  = {2016},
 booktitle = {International Conference on Machine Learning}
}

@book{cover_thomas,
 author = {Thomas M. Cover and Joy A. Thomas},
 title = {Elements of Information Theory},
 publisher = {Wiley-Interscience},
 year = 2006
}
 






@inproceedings{otke,
  title = {A Trainable Optimal Transport Embedding for Feature Aggregation and its Relationship to Attention},
  author = {Gr\'{e}goire Mialon and Dexiong Chen and Alexandre d'Aspremont and Julien Mairal},
  booktitle = {International Conference on Learning Representations},
  year = {2021}
}

@Book{ot_villani,
  author = 	 "Villani, C\'{e}dric",
  title = 	 "Optimal Transport: Old and New",
  publisher = 	 "Springer",
  year = 	 "2008",
}

@inproceedings{ot_cuturi,
  title={{Sinkhorn Distances: Lightspeed Computation of Optimal Transportation Distances}},
  author={Marco Cuturi},
  booktitle={Advances in Neural Information Processing Systems},
  year={2013}
}

@inproceedings{transformer,
  title={Attention Is All You Need},
  author={Ashish Vaswani and Noam Shazeer and Niki Parmar and Jakob Uszkoreit and Llion Jones and Aidan N. Gomez and Lukasz Kaiser and Illia Polosukhin},
  booktitle={Advances in Neural Information Processing Systems},
  year={2017}
}

@article{emd_kernel,
  title={The Earth Mover's Distance as a Metric for Image Retrieval},
  author={Yossi Rubner and Carlo Tomasi and Leonidas J. Guibas},
  journal={International Journal of Computer Vision},
  year={2000},
  volume = {40},
  pages = {99--121}
}

@article{comp_ot,
  title={Computational optimal transport},
  author={Gabriel Peyre and Marco Cuturi},
  journal={Foundations and Trends in Machine Learning},
  year={2019},
  volume = {11},
  number = {5-6},
  pages = {355--206}
}


@Book{kernel_book,
  author = {Bernhard Sch\"{o}lkopf and Alexander J. Smola},
  title = {Learning with Kernels},
  publisher = {MIT Press, Cambridge},
  year = {2002},
}

@article{deepsf,
  title={{DeepSF: Deep convolutional neural network for mapping protein sequences to folds}},
  author={Jie Hou and Badri Adhikari and Jianlin Cheng},
  journal={Bioinformatics},
  year={2019},
  volume = {34},
  number = {8},
  pages = {1295--1303}
}

@article{ckn,
  title={{Biological sequence modeling with convolutional kernel networks}},
  author={Dexiong Chen and Laurent Jacob and Julien Mairal},
  journal={Bioinformatics},
  year={2019},
  volume = {35},
  number = {18},
  pages = {3294--3302}
}

@inproceedings{rkn,
  title={Recurrent kernel networks},
  author={Dexiong Chen and Laurent Jacob and Julien Mairal},
  booktitle={Advances in Neural Information Processing Systems},
  year={2019}
}

@misc{rep_the_set,
 author = {Konstantinos Skianis and Giannis Nikolentzos and Stratis Limnios and Michalis Vazirgiannis},
 title = {{Rep the set: Neural networks for learning set representations}},
 note = {AI and Statistics (AISTATS)},
 year = 2020
}

@inproceedings{nystrom,
  title={{Using the Nystr\"{o}m method to speed up kernel machines}},
  author={Christopher K. I. Williams and Matthias Seeger},
  booktitle={Advances in Neural Information Processing Systems},
  year={2001}
}

@InProceedings{set_transformer,
    title={Set Transformer: A Framework for Attention-based Permutation-Invariant Neural Networks},
    author={Lee, Juho and Lee, Yoonho and Kim, Jungtaek and Kosiorek, Adam and Choi, Seungjin and Teh, Yee Whye},
    booktitle={Proceedings of the 36th International Conference on Machine Learning},
    pages={3744--3753},
    year={2019}
}




@Book{bishop:2006:PRML,
  author = 	 "Christopher M. Bishop",
  title = 	 "Pattern Recognition and Machine Learning",
  publisher = 	 "Springer",
  year = 	 "2006",
}

@article{metaqda,
  title={{Shallow Bayesian Meta Learning for Real-World Few-Shot Recognition}},
  author={Xueting Zhang and Debin Meng and Henry Gouk and Timothy Hospedales},
  journal={arXiv preprint arXiv:2101.02833},
  year={2021}
}

@inproceedings{gpdkt,
  title={Bayesian Meta-Learning for the Few-Shot Setting via Deep Kernels},
  author={Patacchiola, Massimiliano and Turner, Jack and Crowley, Elliot J. and Storkey, Amos},
  booktitle={Advances in Neural Information Processing Systems},
  year={2020}
}

@misc{dkl16,
 author = {Andrew Gordon Wilson and Zhiting Hu and Ruslan Salakhutdinov and Eric P. Xing},
 title = {Deep Kernel Learning},
 note = {AI and Statistics (AISTATS)},
 year = 2016
}

@article{simpleshot,
  title={SimpleShot: Revisiting Nearest-Neighbor Classification for Few-Shot Learning},
  author={Wang, Yan and Chao, Wei-Lun and Weinberger, Kilian Q.  and van der Maaten, Laurens},
  journal={arXiv preprint arXiv:1911.04623},
  year={2019}
}







@inproceedings{nguyen2018variational,
  title = {Variational Continual Learning},
  author = {Nguyen, Cuong V. and Li, Yingzhen and Bui, Thang D. and Turner, Richard E.},
  booktitle = {International Conference on Learning Representations},
  year = {2018}
}



@inproceedings{neural_statistician,
  title = {Towards a Neural Statistician},
  author = {Harrison Edwards and Amos Storkey},
  booktitle = {International Conference on Learning Representations},
  year = {2017}
}

@InProceedings{pa_cvpr20,
  author = {Kim, Sungyeon and Kim, Dongwon and Cho, Minsu and Kwak, Suha},
  title = {Proxy Anchor Loss for Deep Metric Learning},
  booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  month = {June},
  year = {2020}
}

@Article{he2019moco,
  author  = {Kaiming He and Haoqi Fan and Yuxin Wu and Saining Xie and Ross Girshick},
  title   = {Momentum Contrast for Unsupervised Visual Representation Learning},
  journal = {arXiv preprint arXiv:1911.05722},
  year    = {2019},
}



@misc{adam,
 author = {D. P. Kingma and L. J. Ba},
 title = {{Adam: A Method for Stochastic Optimization}},
 note = {{International Conference on Learning Representations (ICLR)}},
 year = 2015
}



@article{kmeans,
 author = {J. Wang and J. Wang and J. Song and X. Xu and H. Shen and S. Li},
 title = {Optimized cartesian k-means},
 journal = {IEEE Transactions on Knowledge and Data Engineering},
 year = {2015},
 volume = {27},
 number = {1},
 pages = {180--192}
}


@manual{mpmath,
  key     = {mpmath},
  author  = {Fredrik Johansson and others},
  title   = {mpmath: a {P}ython library for arbitrary-precision floating-point arithmetic (version 0.18)},
  note    = {{\tt http://mpmath.org/}},
  month   = {December},
  year    = {2013},
}

@article{banerjee05,
 author = {Arindam Banerjee and Inderjit S. Dhillon and Joydeep Ghosh and Suvrit Sra},
 title = {Clustering on the Unit Hypersphere using von Mises-Fisher Distributions},
 journal = {Journal of Machine Learning Research},
 year = {2005},
 volume = {6},
 pages = {1345--1382}
}

@article{s-vae18,
  title={Hyperspherical Variational Auto-Encoders},
  author={Davidson, Tim R. and
          Falorsi, Luca and
          De Cao, Nicola and
          Kipf, Thomas and
          Tomczak, Jakub M.},
  journal={34th Conference on Uncertainty in Artificial Intelligence (UAI-18)},
  year={2018}
}

@article{vmf_samp,
 author = {Gary Ulrich},
 title = {Computer Generation of Distributions on the m-Sphere},
 journal = {Journal of the Royal Statistical Society. Series C (Applied Statistics)},
 year = {1984},
 volume = {33},
 number = {2},
 pages = {158--163}
}

@article{sem,
 author = {Olivier Capp\'{e} and Eric Moulines},
 title = {On-Line Expectation-Maximization Algorithm for Latent Data Models},
 journal = {Journal of the Royal Statistical Society. Series B (Statistical Methodology)},
 year = {2009},
 volume = {71},
 number = {3},
 pages = {593--613}
}

@misc{sem_var,
 author = {Jianfei Chen and Jun Zhu and Yee Whye Teh and Tong Zhang},
 title = {Stochastic Expectation Maximization with Variance Reduction},
 note = {In Advances in Neural Information Processing Systems},
 year = 2018
}

@article{em77,
 author = {A. P. Dempster and N. M. Laird and D. B. Rubin},
 title = {Maximum Likelihood from Incomplete Data via the EM Algorithm},
 journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
 year = {1977},
 volume = {39},
 number = {1},
 pages = {1--38}
}

@article{robbins_monro,
 author = {Herbert Robbins and Sutton Monro},
 title = {A Stochastic Approximation Method},
 journal = {Annals of Mathematical Statistics},
 year = {1951},
 volume = {22},
 number = {3},
 pages = {400--407}
}
    








@inproceedings{wrn,
  title = {{Wide residual networks}},
  booktitle = {BMVC},
  year = {2016},
  author = {Zagoruyko, S. and Komodakis, N.}
}


@misc{funcgrad_friedman,
 author = {Friedman, J.},
 title = {Greedy function approximation: {A} gradient boosting machine},
 note = {Technical Report, Dept. of Statistics, Stanford University.},
 year = 1999
}

@book{funcgrad_mason,
 author = {Mason, L. and Baxter, J. and Bartlett, P. and Frean, M.},
 title = {Functional gradient techniques for combining hypotheses},
 publisher = {In Advances in Large Margin Classifiers, MIT Press},
 year = 1999
}



@article{hmoe,
 author = {M. I. Jordan and R. A. Jacobs},
 title = {Hierarchical mixtures of experts and the {EM} algorithm},
 journal = {Neural Computation},
 year = {1994},
 volume = {6},
 number = {2},
 pages = {181--214}
}

@inproceedings{bhmoe,
 title = {Bayesian hierarchical mixtures of experts},
 author  = {C. M. Bishop and M. Svensen},
 year  = {2003},
 booktitle = {Uncertainty in Artificial Intelligence}
}

@inproceedings{hessian_domke,
 title = {Generic Methods for Optimization-based Modeling},
 author  = {Domke, Justin},
 year  = {2012},
 booktitle = {Artificial Intelligence and Statistics}
}

@misc{hessian_lecun,
 author = {LeCun, Yann and Simard, Patrice and Pearlmutter, Barak},
 title = {Automatic Learning Rate Maximization by On-line Estimation of
the Hessians Eigenvectors},
 note = {In Advances in Neural Information Processing Systems},
 year = 1993
}

@inproceedings{maml,
 title = {Model-Agnostic Meta-Learning for Fast Adaptation of Deep Networks},
 author  = {Chelsea Finn and Pieter Abbeel and Sergey Levine},
 year  = {2017},
 booktitle = {International Conference on Machine Learning}
}

@inproceedings{vlae,
 title = {Variational Laplace Autoencoders},
 author  = {Yookoon Park and Chris Kim and Gunhee Kim},
 year  = {2019},
 booktitle = {International Conference on Machine Learning}
}

@inproceedings{savae_krishnan,
 title = {On the challenges of learning with inference networks on sparse high-dimensional data},
 author  = {Krishnan, R. G. and Liang, D. and Hoffman, M. D.},
 year  = {2018},
 booktitle = {Artificial Intelligence and Statistics}
}

@inproceedings{savae_marino,
 title = {Iterative amortized inference},
 author  = {Marino, J. and Yisong, Y. and Mandt, S.},
 year  = {2018},
 booktitle = {International Conference on Machine Learning}
}

@inproceedings{savae_ykim,
 title = {Semi-amortized variational autoencoders},
 author  = {Kim, Y. and Wiseman, S. and Millter, A. C. and Sontag, D. and Rush,
A. M.},
 year  = {2018},
 booktitle = {International Conference on Machine Learning}
}

@inproceedings{cremer18,
 title = {Inference Suboptimality in Variational Autoencoders},
 author  = {Chris Cremer and Xuechen Li and David Duvenaud},
 year  = {2018},
 booktitle = {International Conference on Machine Learning}
}

@article{svi,
 author = {Hoffman, Matthew D. and Blei, David M. and Wang, Chong and Paisley,
John},
 title = {Stochastic Variational Inference},
 journal = {Journal of Machine Learning Research},
 year = {2013},
 volume = {13},
 pages = {1303--1347}
}


@inproceedings{adversarial_kl,
 title = {An Alternative Update Rule for Generative Adversarial Networks},
 author  = {Ferenc Husz\'{a}r},
 year  = {2016},
 URL = {http://www.inference.vc/an-alternative-update-rule-for-generative-adversarial-networks/},
 booktitle = {Personal blog post}
}

@misc{mirror_vae,
 title = {Enforcing Disentanglement of Latent Factors: Mirror-Factor {VAE}},
 author  = {Minyoung Kim and Vladimir Pavlovic},
 year  = {2018},
 note = {Unpublished manuscript}
}

@inproceedings{nica17,
 title = {Learning independent features with adversarial nets for non-linear {ICA}},
 author  = {Brakel, P. and Bengio, Y.},
 year  = {2017},
 URL = {https://arxiv.org/abs/1710.05050},
 booktitle = {arXiv preprint}
}

@inproceedings{inv_ae,
 title = {Invertible Autoencoder for domain adaptation},
 author  = {Yunfei Teng and Anna Choromanska and Mariusz Bojarski},
 year  = {2018},
 URL = {https://arxiv.org/abs/1802.06869},
 booktitle = {arXiv preprint}
}

@inproceedings{sdae,
 title = {Extracting and Composing Robust Features with Denoising Autoencoders},
 author  = {P. Vincent and H. Larochelle and Y. Bengio and P.A. Manzagol},
 year  = {2008},
 booktitle = {Proceedings of the Twenty-fifth International Conference on Machine Learning}
}


@book{ica_book,
 author = {A. Hyv\"{a}rinen and J. Karhunen and E. Oja},
 title = {Independent Component Analysis},
 publisher = {John Wiley \& Sons, New York},
 year = 2001
}

@article{fast_ica,
 author = {A. Hyv\"{a}rinen and E. Oja},
 title = {A fast fixed point algorithm for independent component analysis},
 journal = {Neural Computation},
 year = {1997},
 volume = {9},
 number = {7},
 pages = {1483--1492}
}

@book{semi_param_book,
 author = {P. J. Bickel and C. A. J. Klaassen and Y. Ritov and J. A. Wellner},
 title = {Efficient and Adaptive Estimation for Semiparametric Models},
 publisher = {Springer-Verlag, New York},
 year = 1998
}

@article{kernel_ica,
 author = {F. Bach and M. I. Jordan},
 title = {Kernel independent component analysis},
 journal = {Journal of Machine Learning Research},
 year = {2002},
 volume = {3},
 pages = {1--48}
}

@misc{amari_ica,
 author = {S. Amari and A. Cichocki and H. H. Yang},
 title = {A new learning algorithm for blind signal separation},
 note = {In Advances in Neural Information Processing Systems},
 year = 1996
}

@article{comon_ica,
 author = {P. Comon},
 title = {{Independent component analysis, A new concept?}},
 journal = {Signal Processing},
 year = {1994},
 volume = {36},
 number = {3},
 pages = {287--314}
}

@inproceedings{matchingnet,
  title={Matching Networks for One Shot Learning},
  author={Oriol Vinyals and Charles Blundell and Timothy Lillicrap and Koray Kavukcuoglu and Daan Wierstra},
  booktitle={Advances in Neural Information Processing Systems},
  year={2016}
}

@inproceedings{reptile,
  title = {{On First-Order Meta-Learning Algorithms}},
  author = {Alex Nichol and Joshua Achiam and John Schulman},
  booktitle = {arXiv preprint arXiv:1803.02999},
  year = {2018}
}

@article{density_ratio_jordan,
 author = {Nguyen, X. and Wainwright, M. J. and Jordan, M. I.},
 title = {Estimating divergence functionals and the likelihood ratio by convex risk minimization},
 journal = {IEEE Transactions on Information Theory},
 year = {2010},
 volume = {56},
 number = {11},
 pages = {5847--5861}
}

@article{density_ratio_sugiyama,
 author = {Sugiyama, M. and Suzuki, T. and Kanamori, T.},
 title = {Density-ratio matching under the {Bregman} divergence: {A} unified framework of density-ratio estimation},
 journal = {Annals of the Institute of Statistical Mathematics},
 year = {2012},
 volume = {64},
 number = {5},
 pages = {1009--1044}
}

@misc{gan,
 author = {Goodfellow, I. and Pouget-Abadie, J. and Mirza, M. and Xu, B. and Warde-Farley, D. and Ozair, S. and Courville, A. and Bengio, Y.},
 title = {Generative Adversarial Nets},
 note = {In Advances in Neural Information Processing Systems},
 year = 2014
}




@misc{vae14,
 author = {Kingma, Diederik P. and Welling, Max},
 title = {Auto-Encoding Variational {B}ayes},
 note = {In Proceedings of the Second International
Conference on Learning Representations, ICLR},
 year = 2014
}

@inproceedings{aae16,
 title = {Adversarial Autoencoders},
 author  = {Alireza Makhzani and Jonathon Shlens and Navdeep Jaitly and Ian Goodfellow and Brendan Frey},
 year  = {2016},
 URL = {http://arxiv.org/abs/1511.05644},
 booktitle = {International Conference on Learning Representations}
}

@unpublished{factor_vae18,
  author = {Kim, H. and Mnih, A.},
  note = {ArXiv e-prints: arXiv:1802.05983},
  title = {Disentangling by Factorising},
  year = {2018}
}

@inproceedings{beta_vae17,
 title = {{Beta-VAE}: Learning basic visual concepts with a constrained variational framework.},
 author  = {Higgins, I. and Matthey, L. and Pal, A. and Burgess, C. and Glorot, X. and Botvinick, M. and Mohamed, S. and Lerchner, A.},
 year  = {2017},
 booktitle = {International Conference on Learning Representations}
}

@inproceedings{dip_vae18,
 title = {Variation inference of disentangled latent concepts from unlabeled observations},
 author  = {Kumar, A. and Sattigeri, P. and Balakrishnan, A},
 year  = {2018},
 booktitle = {International Conference on Learning Representations}
}

@misc{infogan16,
 author = {Chen, X. and Duan, Y. and Houthooft, R. and Schulman, J. and Sutskever, I. and Abbeel, P.},
 title = {{InfoGAN: Interpretable representation learning by information maximizing Generative Adversarial Nets}},
 note = {In Advances in Neural Information Processing Systems},
 year = 2016
}

@inproceedings{dsprites,
 title = {{dSprites: Disentanglement testing Sprites dataset}},
 author  = {Matthey, L. and Higgins, I. and Hassabis, D. and Lerchner, A.},
 year  = {2017},
 URL = {https://github.com/deepmind/dsprites-dataset/},
 booktitle = {}
}










@inproceedings{DuvMacetal15nfp,
	booktitle = {Neural Information Processing Systems},
	title     = {Convolutional Networks on Graphs for Learning Molecular Fingerprints},
	author    = {David Duvenaud and Dougal Maclaurin and Jorge Aguilera-Iparraguirre and Rafael G\'omez-Bombarelli and Timothy Hirzel and Al\'an Aspuru-Guzik and Ryan P. Adams},
	year      = {2015}
}

@misc{rfdnn17,
 author = {K. Cutajar and E. V. Bonilla and P. Michiardi and M. Filippone},
 title = {Random Feature Expansions for Deep {G}aussian Processes},
 note = {International Conference on Machine Learning},
 year = 2017
}

@misc{deepgp13,
 author = {Damianou, Andreas C. and Lawrence, Neil D.},
 title = {Deep {G}aussian Processes},
 note = {In Proceedings of the Sixteenth International
Conference on Artificial Intelligence and Statistics},
 year = 2013
}

@misc{rf_arccos,
 author = {Cho, Youngmin and Saul, Lawrence K.},
 title = {Kernel methods for deep learning},
 note = {In Advances in Neural Information Processing Systems},
 year = 2009
}

@misc{rf_fourier,
 author = {Rahimi, Ali and Recht, Benjamin},
 title = {Random Features for Large-Scale Kernel Machines},
 note = {In Platt, J. C., Koller, D., Singer, Y., and Roweis, S. T. (eds.), 
Advances in Neural Information Processing Systems 20},
 year = 2008
}

@book{rudin_book,
 author = {W. Rudin},
 title = {Fourier Analysis on Groups. Wiley Classics Library},
 publisher = {Wiley-Interscience, New York},
 year = 1994
}

@book{gpml_book,
 author = {Carl Edward Rasmussen and Christopher K. I. Williams},
 title = {Gaussian Processes for Machine Learning},
 publisher = {The MIT Press},
 year = 2006
}

@misc{titsias09,
 author = {M. K. Titsias},
 title = {Variational Learning of Inducing Variables in Sparse {G}aussian Processes},
 note = {In Proceedings of the Twelfth International Conference on 
Artificial Intelligence and Statistics},
 year = 2009
}

@misc{dezfouli15,
 author = {A. Dezfouli and E. V. Bonilla},
 title = {Scalable Inference for {G}aussian Process Models with Black-Box Likelihoods},
 note = {In Advances in Neural Information Processing Systems},
 year = 2015
}










@misc{gpmil_icml10,
 author = {Minyoung Kim and Fernando {De la Torre}},
 title = {Gaussian Process Multiple Instance Learning},
 note = {International Conference on Machine Learning},
 year = 2010
}

@article{Dietterich97,
 author = {Thomas G. Dietterich and Richard H. Lathrop and Tomas Lozano-Perez},
 title = {Solving the Multiple-Instance Problem with Axis-Parallel Rectangles},
 journal = {Artificial Intelligence},
 year = {1997},
 volume = {89},
 pages = {31--71}
}

@article{mil_real,
 author = {Daniel R. Dooly and Qi Zhang and Sally A. Goldman and Robert A. Amar},
 title = {Multiple-Instance Learning of Real-Valued Data},
 journal = {Journal of Machine Learning Research},
 year = {2002},
 volume = {3},
 pages = {651--678}
}

@misc{mik02,
 author = {Thomas G\"{a}rtner and Peter A. Flach and Adam Kowalczyk and Alex J. Smola},
 title = {Multi-Instance Kernels},
 note = {International Conference on Machine Learning},
 year = 2002
}

@misc{hausdorff00,
 author = {Jun Wang and Jean-Daniel Zucker},
 title = {Solving the Multiple-Instance Problem: {A} Lazy Learning Approach},
 note = {International Conference on Machine Learning},
 year = 2000
}

@misc{bmil08,
 author = {Vikas C. Raykar and Balaji Krishnapuram and Jinbo Bi and Murat Dundar and R. Bharat Rao},
 title = {Bayesian multiple instance learning: {A}utomatic feature selection and inductive transfer},
 note = {International Conference on Machine Learning},
 year = 2008
}

@misc{missl06,
 author = {Rouhollah Rahmani and Sally A. Goldman},
 title = {{MISSL: M}ultiple-Instance Semi-Supervised Learning},
 note = {International Conference on Machine Learning},
 year = 2006
}

@misc{ihs05,
 author = {Zhang, H. and Fritts, J.},
 title = {Improved hierarchical segmentation},
 note = {{Technical Report, Washington University in St Louis}},
 year = 2005
}

@misc{pets,
 author = {O. M. Parkhi and A. Vedaldi and A. Zisserman and C. V. Jawahar},
 title = {{Cats and Dogs}},
 note = {{IEEE Conference on Computer Vision and Pattern Recognition}},
 year = 2012
}

@misc{flowers,
 author = {Nilsback, M-E. and Zisserman, A.},
 title = {{Automated flower classification over a large number of classes}},
 note = {{Proceedings of the Indian Conference on Computer Vision, Graphics and Image Processing}},
 year = 2008
}


@inproceedings{liegroup,
  title = {{Reparameterizing distributions on Lie groups}},
  author = {Falorsi, L. and de Haan, P. and Davidson, T. R. and Forr\'{e}, P.},
  booktitle = {arXiv preprint arXiv:1903.02958},
  year = {2019}
}



@misc{invar1,
 author = {Laptev, D. and Savinov, N. and Buhmann, J. M. and Pollefeys, M.},
 title = {{Ti-pooling: Transformation-invariant pooling for feature learning in convolutional neural networks}},
 note = {{IEEE conference on computer vision and pattern recognition}},
 year = 2016
}

@misc{invar2,
 author = {Raj, A. and Kumar, A. and Mroueh, Y. and Fletcher, T. and Sch\"{o}lkopf, B.},
 title = {{Local group invariant representations via orbit embeddings}},
 note = {{Artificial Intelligence and Statistics}},
 year = 2017
}

@misc{invar3,
 author = {van der Wilk, M. and Bauer, M. and John, S. and Hensman, J.},
 title = {{Learning invariances using the marginal likelihood}},
 note = {{In Advances in Neural Information Processing Systems}},
 year = 2018
}


@article{miles06,
 author = {Yixin Chen and Jinbo Bi and J. Z. Wang},
 title = {{MILES}: {M}ultiple-Instance Learning via Embedded Instance Selection},
 journal = {IEEE Trans. on Pattern Analysis and Machine Intelligence},
 year = {2006},
 volume = {28},
 number = {12},
 pages = {1931--1947}
}

@misc{dd98,
 author = {Oded Maron and Tomas Lozano-Perez},
 title = {A Framework for Multiple-Instance Learning},
 note = {Neural Information Processing Systems},
 year = 1998
}

@misc{tao04,
 author = {Qingping Tao and Stephen Scott and N. V. Vinodchandran and Thomas Takeo Osugi},
 title = {{SVM}-Based Generalized Multiple-Instance Learning via Approximate Box Counting},
 note = {International Conference on Machine Learning},
 year = 2004
}

@misc{emdd,
 author = {Qi Zhang and Sally A. Goldman and Wei Yu and Jason E. Fritts},
 title = {Content-Based Image Retrieval Using Multiple-Instance Learning},
 note = {International Conference on Machine Learning},
 year = 2002
}

@article{mica,
 author = {O. L. Mangasarian and E. W. Wild},
 title = {Multiple Instance Classification via Successive Linear Programming},
 journal = {Journal of Optimization Theory and Applications },
 year = {2008},
 volume = {137},
 number = {3},
 pages = {555--568}
}

@misc{mil_boost05,
 author = {Paul A. Viola and John C. Platt and Cha Zhang},
 title = {Multiple Instance Boosting for Object Detection},
 note = {Neural Information Processing Systems},
 year = 2005
}

@misc{mil_svm03,
 author = {Stuart Andrews and Ioannis Tsochantaridis and Thomas Hofmann},
 title = {Support vector machines for multiple-instance learning},
 note = {Neural Information Processing Systems},
 year = 2003
}

@misc{mil_da07,
 author = {Peter V. Gehler and Olivier Chapelle},
 title = {Deterministic Annealing for Multiple-Instance Learning},
 note = {AI and Statistics (AISTATS)},
 year = 2007
}

@misc{semisup_gpc07,
 author = {Vikas Sindhwani and Wei Chu and S. S. Keerthi},
 title = {Semi-Supervised {G}aussian Process Classifiers},
 note = {International Joint Conferences on Artificial Intelligence (IJCAI)},
 year = {2007},
}

@misc{semisup_kernel05,
 author = {Vikas Sindhwani and Partha Niyogi and M. Belkin},
 title = {Beyond the point cloud: {F}rom transductive to semi-supervised learning},
 note = {International Conference on Machine Learning},
 year = {2005},
}

@misc{bennett00,
 author = {Ayhan Demiriz and Kristin P. Bennett},
 title = {Optimization Approaches to Semi-Supervised Learning},
 note = {Applications and Algorithms of Complementarity},
 year = {2000}
}

@misc{joachims99,
 author = {Thorsten Joachims},
 title = {Transductive Inference for Text Classification using Support Vector Machines},
 note = {International Conference on Machine Learning},
 year = {1999},
}

@misc{Friedman99,
 author = {J. Friedman},
 title = {Greedy Function Approximation: a Gradient Boosting Machine},
 note = {Technical Report, Dept. of Statistics, Stanford University},
 year = 1999,
}




@article{emep,
 author = {Hyun-Chul Kim and Zoubin Ghahramani},
 title = {{B}ayesian {G}aussian Process Classification with the {EM-EP} Algorithm},
 journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
 volume = 28,
 number = 12,  
 pages = {1948--1959}, 
 year = 2006
}

@misc{cvx_a,
 author = {M. Grant and S. Boyd},
 title = {{CVX}: {Matlab} software for disciplined convex programming (web page and software)},
 note = {http://stanford.edu/~boyd/cvx},
 year = 2009
}

@misc{cvx_b,
 author = {M. Grant and S. Boyd},
 title = {Graph implementations for nonsmooth convex programs},
 note = {Recent Advances in Learning and Control (a tribute to M. Vidyasagar), V. Blondel, S. Boyd, and H. Kimura, editors, pages 95-110, Lecture Notes in Control and Information Sciences, Springer},
 year = 2008
}

@book{wilcoxon,
 author = {Hollander, M. and D. A. Wolfe},
 title = {Nonparametric Statistical Methods},
 publisher = {Wiley},
 year = 1973
}



@article{zhang01,
 author = {Tong Zhang and Frank J. Oles},
 title = {Text Categorization Based on Regularized Linear Classification Methods},
 journal = {Information Retrieval},
 volume = {4},
 pages = {5--31},
 year = 2000
}

@misc{ep,
 author = {Thomas Minka},
 title = {A family of algorithms for approximate {B}ayesian inference},
 note = {MIT PhD thesis},
 year = 2001
}

@misc{ep_gpc,
 author = {Matthias Seeger},
 title = {Notes on {M}inka's Expectation Propagation for {G}aussian process classification},
 note = {Technical Report, University of Edinburgh},
 year = 2002
}





